Visual Discovery at Pinterest

Over the past three years Pinterest has experimented with several visual search and recommendation services, including Related Pins (2014), Similar Looks (2015), Flashlight (2016) and Lens (2017). This paper presents an overview of our visual discovery engine powering these services, and shares the rationales behind our technical and product decisions such as the use of object detection and interactive user interfaces. We conclude that this visual discovery engine significantly improves engagement in both search and recommendation tasks.

==> 2.3-incremental.tex <==
\subsection{Incremental Fingerprinting Service}

\label{sec:incremental}



\label{sec:ifs}
Most of our vision applications depend on having a complete collection of image features, stored in a format amenable to bulk processing.
Keeping this data up-to-date is challenging; because
%many new images are added every day, and we continually add and modify features for new applications. Since
our collection comprises over a billion unique images, it is critical to update the feature set incrementally and avoid unnecessary re-computation whenever possible.

% There are several practical challenges associated with maintaining and updating this set of features.
% First, Pinterest has more than one billion unique images, so we want to avoid unnecessary re-computation for existing images when updating the collection.
% Second, a large number of images are added to the database every day, and we want to incorporate the features of new images within a reasonable time frame.\footnote{Image features needed in real-time are handled by a separate service.}
% Third, we continue to add and refine features for new applications, while most older features remain unchanged. We want to compute new or modified features while avoiding redundant computation of unchanged features.

%Using largely open-source software and platforms, we built a system to scale feature computation to handle over one billion images.  Specifically, we introduce a cost-effective distributed processing platform that supports incremental updates.

We built a system called the \textit{Incremental Fingerprinting Service}, which computes image features for all Pinterest images using a cluster of workers on Amazon EC2. It incrementally updates the collection of features under two main change scenarios: new images uploaded to Pinterest, and feature evolution (features added/modified by engineers).

%\begin{figure}
%\centering
%\includegraphics[height=7 in]{images/ifu_2}
%\caption{Examples of outputs generated by incremental fingerprint update pipeline. The initial run is shown as 2014-xx-xx which includes all %the images created before that run.}
%\label{fig:ifu_2}
%\end{figure}



Our approach is to split the image collection into \textit{epochs} grouped by upload date, and to maintain a separate feature store for each version of each feature type (global, local, deep features). Features are stored in bulk on Amazon S3, organized by feature type, version, and date. %Each file holds features of a particular type for about 200,000 images, stored in length-delimited Google Protocol Buffers.
When the data is fully up-to-date, each feature store contains all the epochs. On each run, the system detects missing epochs for each feature and enqueues jobs into a distributed queue to populate those epochs.

%Only a portion of the epochs and features are updated during each run of the system, and the results are merged with the unchanged epochs.

This storage scheme enables incremental updates as follows. Every day, a new epoch is added to our collection with that day's unique uploads, and we generate the missing features for that date. Since old images do not change, their features are not recomputed.  If the algorithm or parameters for generating a feature are modified, or if a new feature is added, a new feature store is started and all of the epochs are computed for that feature.  Unchanged features are not affected.

We copy these features into various forms for more convenient access by other jobs: features are merged to form a \textit{fingerprint} containing all available features of an image, and fingerprints are copied into sharded, sorted files for random access by image signature (MD5 hash). These joined fingerprint files are regularly re-materialized, but the expensive feature computation needs only be done once per image.

The incremental fingerprint update process consists of five main jobs:  job (1) compiles a list of newly uploaded image signatures and groups them by date into epochs. We randomly divide each epoch into sorted shards of approximately 200,000 images to limit the size of the final fingerprint files.  Job (2) identifies missing epochs in each feature store and enqueues jobs into PinLater (a distributed queue service similar to Amazon SQS). The jobs subdivide the shards into ``work chunks", tuned such that each chunk takes approximate 30 minutes to compute.
Job (3) runs on an automatically-launched cluster of EC2 instances, scaled depending on the size of the update. Spot instances can be used; if an instance is terminated, its job is rescheduled on another worker. The output of each work chunk is saved onto S3, and eventually recombined into feature files corresponding to the original shards.

Job (4) merges the individual feature shards into a unified fingerprint containing all of the available features for each image. Job (5) merges fingerprints from all epochs (along with other metadata) into a sorted, sharded HFile format allowing for random access \textit{(VisualJoins)}.

The initial computation of all available features on all images, takes a little over a day using a cluster of several hundred 32-core machines, and produces roughly 5~TB of feature data.  The steady-state requirement to process new images incrementally is only about 5 machines.

% Optional - dliu: this is not that interesting.
%As expected, feature computation completely dominates the runtime. Merging individual features into fingerprints takes only a few minutes per date epoch, and further batch jobs are limited only by S3 transfer speed: the production Hadoop cluster can comfortably read all fingerprints in about 20 minutes.

==> 2.4-search.tex <==
\subsection{Search Infrastructure}
%TODO: refresh diagram with better one. talk about asynchronous collator. 

At Pinterest, there are several use cases for a distributed visual search system.  One use case is to explore similar looking objects (Section~\ref{productsearch}), and others include near-duplicate detection and content recommendation (Section~\ref{sec:app-related-pins}). In all these applications, visually similar results are computed from distributed indices built on top of the VisualJoin features generated in the previous section. Since each use case has a different set of performance and cost requirements, our infrastructure is designed to be flexible and re-configurable.  A flow chart of the search infrastructure is shown in Figure~\ref{fig:search_pipeline}.



\begin{figure}
	\centering
	\includegraphics[width=3.2in]{images/search_pipeline_2}
	\caption{A flow chart of the distributed visual search pipeline.}
	\label{fig:search_pipeline}
\end{figure}

As the first step we create distributed image indices from VisualJoins using Hadoop.  Each machine contains indexes (and features) associated with a randomly sharded subset of the entire image collection.  Two types of indexes are used: the first is a disk-based (and partially memory cached) \textit{token index} associating each vector-quantized feature (i.e. visual vocabulary token) with a posting list of image document IDs. This is analogous to a text-based image retrieval system, except text is replaced by visual tokens. The second index is an in-memory store of visual features and metadata such as image annotations and ``topic vectors'' computed from the user-board-image graph.
For both versions, the fast (but imprecise) index lookup is used to generate visual candidates while the metadata along with the visual features are used for more accurate (but slower) ranking refinement of the candidates.
%The first part is used for fast (but imprecise) lookup, and the second part is used for more accurate (but slower) ranking refinement.   %%%%%%%%% dliu: this is ambiguous. does "first, second part" mean token index + in-memory store or does it mean the visual features and metadata? It's got to mean the latter, because in-memory is way faster than disk.

Each machine runs a leaf ranker, which computes the $k$ nearest neighbors from the indices using visual features, and then re-ranks the top candidates using additional metadata. In some cases, the leaf ranker skips the token index and directly retrieves the $k$ nearest neighbor images from the feature tree index using approximate KNN methods such as~\cite{binaryknn}.  A root ranker hosted on another machine will retrieve the top results from each of the leaf rankers, merge the results, and return them to the users. To handle online requests, new fingerprints are generated with our real-time feature extractor while offline requests use the pre-generated fingerprints from VisualJoin.


==> 3.2-similar-looks.tex <==
% SKIP

\section{Case Study 2: Visual Search}
\label{productsearch}

In this section, we detail two visual search experiences. First we discuss \textit{Similar Looks}, an offline, domain-specific detection and retrieval system which was launched at Pinterest in 2014. Similar Looks was ultimately deprecated in favor of a more general, real-time visual search system called \textit{Flashlight}.


\begin{figure}
\centering
\includegraphics[height = 2.5 in]{images/mobileresults}
\caption{Similar Looks: Once a user clicks on the red dot, the system shows products that have a similar appearance to the query object.}
\label{fig:similarlooksmobile}
\end{figure}



\begin{figure*}
	\centering
	\includegraphics[width=5.7 in]{images/flashlight3}
	\caption{Pinterest Flashlight: After pressing on the search icon (Top Left), a user will enter cropping mode and be able to select an object by specifying a region of interest in the image (Top Right). The system then shows Pins that are visually similar to the object along with annotations for the object.  Users can also interact with the annotations to refine the results }
	\label{fig:objectsearchflow_crop}
\end{figure*}



\subsection{Similar Looks}
\label{sec:app-similar-looks}

Similar Looks was a product designed to solve visual search specifically for the fashion category (a popular category on Pinterest). Similar Looks localized and classified visual objects (such as watches, bags, shoes, jackets) using optimized DPMs for detection and an offline retrieval system for finding visually similar products. 

%In \cite{jing15} we introduced Similar Looks, a visual search experiment based on an offline detection and retrieval system. Our focus was to detect 



%One of the most popular categories on Pinterest is women's fashion. However, a large percentage of pins in this category do not direct users to a shopping experience, and therefore are not actionable.  There are two challenges towards making these Pins actionable:
%1) Many pins feature editorial shots such as ``street style'' outfits, which often link to a website with little additional information on the items featured in the image;
%2) Pin images often contain multiple objects (e.g. a woman walking down the street, with a leopard-print bag, black boots, sunglasses, torn jeans, etc.) A user looking at the Pin might be interested in learning more about the bag, while another user might want to buy the sunglasses.

%User research revealed this to be a common frustration, and our data indicated that users are much less likely to click through to the external Website on women's fashion Pins, relative to other categories.


%Figure~\ref{similarlooksmobile} doesn't work, hardcoding figure
%To address this problem, we built a product called ``Similar Looks'', which localizes and classifies fashion objects (Figure~\ref{fig:similarlooksmobile}). We use object recognition to detect products such as bags, shoes, pants, and watches in Pin images. From these objects, we extract visual and semantic features to generate product recommendations (``Similar Looks''). A user would discover the recommendations via a red dot displayed on the object in the Pin (see Figure~\ref{fig:similarlooksmobile}). Clicking on the red dot loads a feed of Pins featuring visually similar objects (e.g. other visually similar blue dresses).
%ence around these detected objects.





%\subsection*{Static Evaluation of Object Localization}

%The first step of evaluating our Similar Looks product was to investigate our object localization and detection capabilities. We chose to focus on fashion objects because of the aforementioned business need and because ``soft goods" tend to have distinctive visual shapes (e.g. shorts, bags, glasses).


%We collected our evaluation dataset by randomly sampling a set of images from Pinterest's women's fashion category, and manually labeling 2,399 fashion objects in 9 categories (shoes, dress, glasses, bag, watch, pants, shorts, bikini, earnings) on the images by drawing a rectangular crop over the objects.  We observed that shoes, bags, dresses and pants were the four largest categories in our evaluation dataset. Shown in Table~\ref{table:objects} is the distribution of fashion objects as well as the detection accuracies from the text-based filter, image-based detection, and the combined approach (where text filters are applied prior to object detection). 


%\label{sec:evaluationobject}
%\begin{table}[h]
%\caption{Object detection/classification accuracy (\%) }

%\label{table:objects}
%\begin{tabular}{  l l | l  l | l l | l l }
%  &  & Text&   &  Img & & Both &   \\
% Objects & \# & TP &  FP  &  TP   & FP  & TP & FP   \\
%\hline
%shoe	 &873&79.8&6.0&41.8&3.1&34.4 &1.0 \\
%dress	&383	&75.5	  &  6.2 &	58.8	& 12.3 & 47.0	& 2.0\\
%glasses	&238	&75.2	& 18.8 & 63.0 & 0.4 &	50.0 &	0.2\\
%bag	&468	&66.2	& 5.3	& 59.8 & 2.9	& 43.6	& 0.5\\
%watch	&36	&55.6	& 6.0	& 66.7 &	0.5	& 41.7	& 0.0\\
%pants	&253	&75.9	 & 2.0	& 60.9	& 2.2	& 48.2	& 0.1\\
%shorts	&89	&73.0	& 10.1 & 44.9 &1.2	& 31.5	& 0.2\\
%bikini	&32	&71.9	& 1.0	& 31.3 &0.2	& 28.1	& 0.0\\
%earrings	&27	&81.5	& 4.7	& 18.5 &0.0	& 18.5	& 0.0\\
%\hline
%Average & & 72.7 & 6.7 & 49.5 & 2.5 & 38.1 & 0.5\\
%\hline
%\end{tabular}
%\end{table}

%As previously described, the text-based approach applies manually crafted rules, such as regular expressions, to the Pinterest metadata associated with images (which we treat as weak labels).  For example, an image annotated with ``spring fashion, \textit{tote} with flowers" will be classified as ``bag," and is considered as a positive sample if the image contains a ``bag" object box label.  For image-based evaluation, we compute the intersection between the predicted object bounding box and the labeled object bounding box of the same type, and count an intersection over union ratio of 0.3 or greater as a positive match.   



%\begin{figure}
%\centering
%\includegraphics[width=3 in]{misc_pos}
%\caption{Recognize objects in bikini, watches and shorts category.}
%\end{figure}

%Table~\ref{table:objects} demonstrates that neither text annotation filters nor object localization alone were sufficient for our detection task due to their relatively high false positive rates at 6.7\% and 2.5\% respectively. Not surprisingly, combining two approaches significantly decreased our false positive rate to less than 1\%.


%Specifically, we saw that for classes like \textit{glasses}, text annotations were insufficient and image-based classification excelled (likely due to the distinctive shape of glasses). For other classes, such as \textit{dress}, this situation was reversed (the false positive rate for our dress detector was high, 12.3\%, due to occlusion and high variance in style for that class, and adding a text filter dramatically improved results). Aside from reducing the number of images we needed to process with our object classifiers, for several object classes (\textit{shoe}, \textit{bag}, \textit{pants}), we observed that text filtering was crucial to achieve an acceptable false positive rate (under 1\%). 


%\subsection*{Live Experiments} 

Our system identified over 80 million ``clickable'' objects from a subset of Pinterest images. A clickable red dot is placed upon the detected object.  Once the user clicks on the dot, our visual search system retrieves a collection of Pins with other instances of the object class, ranked by visually similarity to the query object. We launched the system to a small percentage of Pinterest live traffic and collected user engagement metrics for one month. Specifically, we looked at the clickthrough rate (CTR) of the dot, the CTR on our visual search results, and we compared engagement on Similar Look results with the engagement on existing Related Pins recommendations.



As shown in Figure~\ref{fig:similarlooksresults}, on average, 12\% of users who viewed a pin with a dot clicked on a dot in a given day. Those users went on to click an average of 0.55 Similar Looks results. Although this data was encouraging, when we compared engagement with all related content on the pin close-up (summing both engagement with Related Pins and Similar Look results for the treatment group, and just Related Pins engagement for the control), Similar Looks actually hurt overall engagement on the pin close-up by 4\%. After the novelty effort wore off, we saw a gradual decrease in CTR on the red dots, which stabilized at around 10\%. 

To test the relevance of our Similar Looks results independently of the newly introduced UI (the clickable object dots), we ran an experiment in which we blended Similar Looks results directly into the existing Related Pins. %(for Pins containing detected objects).
This gave us a way to directly measure whether users found our visually similar recommendations more relevant than our existing non-visual recommendations.  On pins where we detected an object, this experiment increased overall engagement (repins and close-ups) in Related Pins by 5\%. Although we set an initial static blending ratio for this experiment (one visually similar result for every three non-visual results), we later adjusted this ratio dynamically using user click data.


\begin{figure}
\centering
\includegraphics[height = 2.5 in]{images/similarlooksresults}
\caption{Engagement rates for Similar Looks experiment}
\label{fig:similarlooksresults}
\end{figure}




% take out the blending ratio altogether? 

%In reviewing these results, our main question was whether it was because of the quality or utility of the results, or because users were slowed down by the new behavior we were trying to introduce with tapping on the dot.  In order to separate these two effects, we designed an experiment where instead of showing a dot on the object, we instead blended the Similar Look Pin results into the existing Related Pins recommendation.  This would let us focus on a clearer evaluation of whether the new recommendations were useful for users. To this end, we tested several different blending rates of Similar Look results and existing related pin results -- specifically, we blended similar look results with the existing related pin results at a ratio of 1:1, 1:2, 1:3 and 2:1. Ultimately, the winning variant was when we mixed in one similar look results for every three existing related pin results. In this treatment, we saw an increase of 5\% more users engage (repin or click) with the Related Pin results.


%\begin{figure}
%\centering
%\includegraphics[width=3.5 in]{images/search_results2}
%\caption{Examples of object search results for shoes. Boundaries of detected objects are automatically %highlighted.  The top image is the query image.}
%\end{figure}


%\begin{figure*}
%\centering
%\includegraphics[width=7 in]{images/bag_pos_small}
%\caption{Samples of object detection and localization results for bags. [Green: ground truth, blue: detected %objects.] }
%\end{figure*}




%\begin{figure*}
%\centering
%\includegraphics[width=7 in]{images/glass_pos_small}
%\caption{Samples of object detection and localization results for glasses}
%\end{figure*}

%\begin{figure*}
%\centering
%\includegraphics[width=6.4 in]{images/dress_pos_small}
%\caption{Samples of object detection and localization results for dresses}
%\end{figure*}
